Distributed Optimal Power Flow Algorithm for Balanced Radial Distribution Networks

The optimal power flow (OPF) problem is fundamental in power system operations and planning. Large-scale renewable penetration in distribution networks calls for real-time feedback control, and hence the need for fast and distributed solutions for OPF. This is difficult because OPF is nonconvex and Kirchhoff's laws are global. In this paper we propose a solution for balanced radial distribution networks. It exploits recent results that suggest solving for a globally optimal solution of OPF over a radial network through the second-order cone program (SOCP) relaxation. Our distributed algorithm is based on alternating direction method of multiplier (ADMM), but unlike standard ADMM algorithms that often require iteratively solving optimization subproblems in each ADMM iteration, our decomposition allows us to derive closed form solutions for these subproblems, greatly speeding up each ADMM iteration. We present simulations on a real-world 2,065-bus distribution network to illustrate the scalability and optimality of the proposed algorithm.

==> texcode/app2.tex <==
\section{Fast algorithm for OPF}

Now we describe another algorithm, which is also based on the decomposition in section \ref{sec:application}. This algorithm cannot be implemented in a distributed manner and has the advantage of faster convergence. For the distributed version, the system dimension is enlarged three times. Here, the new algorithm only enlarge it by twice and does not suffer the problem that the convergence rate depends on the diameter of the graph $\mathG$. 

In this fast algorithm, we only replicate $v,\ell,S,s$ once, denoted by
\bqn
v^{(z)}=v \ \   \ell^{(z)}=\ell \ \ S^{(z)}=S  \ \   s^{(z)}=s
\eqn
and the OPF problem \eqref{eq:ropf} can be written equivalently as 
\begin{subequations}
\bqn
\min && \sum_{i\in \mathN}f_i(p_i)\\
\text{s.t.} && v_{A_i}-v_i+2\mathrm{Re}(\overline z_i S_i)-\ell_{i}|z_{i}|^2=0 \quad i\in \mathN_{-1}  \label{eq:31}\\  
&& \sum_{j\in C_i}(S_{j}-\ell_{j}z_{j})+s_i-S_{i}=0 \quad i\in \mathN   \label{eq:32}\\  
&& z\in\mathcal{K}\\
&&  x=z
\eqn
\end{subequations}

Then in the $x$-update step, the problem required to be solved is
\bqn
\min  && F(v,\ell,S,s)\\
\text{s.t.} &&v_{A_i}-v_i+2\mathrm{Re}(\overline z_i S_i)-\ell_{i}|z_{i}|^2=0 \quad i\in \mathN_{+}  \label{eq:31}\\  
&& \sum_{j\in C_i}(S_{j}-\ell_{j}z_{j})+s_i-S_{i}=0 \quad i\in \mathN   \label{eq:32}
\eqn
where
\begin{align*}
&F(v,\ell,S,s)=\\
&\sum_{i\in \mathN}f_i(p_i)+\lambda_{1}^Tv+\lambda_{2}^T\ell+\lambda_{3}^TS+\lambda_{4}^Ts\\
&\frac{\rho}{2}\left(\|v-v^{(z)}\|_2^2+\|\ell-\ell^{(z)}\|_2^2+\|S-S^{(z)}\|^2+\|s-s^{(z)}\|^2\right)
\end{align*}

The above problem shares the same structure as \eqref{eq:xupdate1} and thus has close form solution. The $z$-update step is the same as the distributed algorithm.


==> texcode/app_no_use.tex <==
\appendices

\section{$4$ variables optimization}

\noindent P1:
\bqn
\min && \sum_{i=1}^4 c_ix_i\\ 
\text{s.t.}&&\underline x_i \leq  x_i\leq \overline x_i \ \ 1\leq i\leq 3 \\
&& x_4\geq 0\\
&& x_3x_4\geq x_1^2+x_2^2
\eqn

Next, we will try to get a close form solution of P1. P1 can be reformulated as:
\bqn
\min_{R\geq 0} f_1(R)+f_2(R)
\eqn
where
\bqn
f_1(R):=\min_{x_1,x_2} \ \ c_1x_1+c_2x_2 \quad s.t. \ \ \underline x_1\leq x_1\leq \overline x_1, \ \underline x_2\leq x_2\leq \overline x_2, \ x_1^2+x_2^2\leq R^2
\eqn
\bqn
f_2(R):=\min_{x_3,x_4} \ \ c_3x_3+c_4x_4 \quad s.t. \ \ \underline x_3\leq x_3\leq \overline x_3, \  x_4\geq 0, \ x_3x_4\geq R^2
\eqn

\begin{table}[htdp]
\caption{The objective value of $f_2(R)$. (Suppose $R^2\leq \overline x_3^2+\overline x_4^2$)}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$c_4$ & $c_3$ & $x_3$ & $x_4$ & Obj ($\overline x_4=\infty$) & Obj \\
\hline 
- & - & $\overline x_3$ & $\overline x_4$ & $-\infty$ & \\
\hline
- & + & $\max\{\underline x_3,\frac{R^2}{\overline x_4}\}$ & $\overline x_4$ & $-\infty$ & \\
\hline
+ & - & $\overline x_3$ & $\frac{R^2}{\overline x_3}$ & $c_3 \overline x_3+c_4\frac{R^2}{\overline x_3}$ & \\
\hline
+ & + & $[R\sqrt{\frac{c_4}{c_3}}]_{\max\{\underline x_3, R^2/\overline x_4\}}^{\overline x_3}$ & Inverse of $x_3$ &
$[2\sqrt{c_3c_4}R]$ ($R\in \sqrt{c_3/c_4}[\underline x_3,\overline x_3]$) &\\
&&&& $c_3\underline x_3+c_4R^2/\underline x_3$ ($R\leq \sqrt{c_3/c_4}\underline x_3$)&\\
&&&& $c_3\overline x_3+c_4R^2/\overline x_3$ ($R\geq \sqrt{c_3/c_4}\overline x_3$)&\\
\hline
\end{tabular}
\end{center}
\label{tab:objf2R}
\end{table}

\begin{table}[htdp]
\caption{The objective value of $f_1(R)$. Suppose $c_1,c_2\geq 0$ and $c_2/c_1\geq \underline x_2/\underline x_1$. Cutoff $\overline x_1=\min\{0,\overline x_1\}$ and $\overline x_2=\min\{0,\overline x_2\}$.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\# of positive vertex $-c_2x_1+c_1x_2$ &$\underline x_1$ & $\underline x_2$& $R^2$ & $x_1$ & $x_2$  & Obj \\
\hline 
$(\underline x_1,\underline x_2)$&- & - & $[\overline x_1^2+\overline x_2^2,\frac{c_1^2+c_2^2}{c_2^2}\overline x_2^2]$ & $-\sqrt{R^2-\overline x_2^2}$ & $\overline x_2$ & $-c_1\sqrt{R^2-\overline x_2^2}+c_2\overline x_2$\\
&- & - & $[\frac{c_1^2+c_2^2}{c_2^2}\overline x_2^2,\frac{c_1^2+c_2^2}{c_2^2}\underline x_2^2]$ & $\frac{-c_1}{\sqrt{c_1^2+c_2^2}}R$ & $\frac{-c_2}{\sqrt{c_1^2+c_2^2}}R$ & $-R\sqrt{c_1^2+c_2^2}$\\
&- & - & $[\frac{c_1^2+c_2^2}{c_2^2}\underline x_2^2, \underline x_1^2+\underline x_2^2]$ & $-\sqrt{R^2-\underline x_2^2}$ & $\underline x_2$ & $c_2 \underline x_2- c_1\sqrt{R^2-\underline x_2^2}$\\
\hline

$(\underline x_1,\underline x_2)$,$(\overline x_1,\overline x_2)$&- & - & $[\overline x_1^2+\overline x_2^2,\frac{c_1^2+c_2^2}{c_1^2}\overline x_1^2]$ & $\overline x_1$ & $-\sqrt{R^2-\overline x_1^2}$ & $c_1\overline x_1-c_2\sqrt{R^2-\overline x_1^2}$\\
&- & - & $[\frac{c_1^2+c_2^2}{c_1^2}\overline x_1^2,\frac{c_1^2+c_2^2}{c_2^2}\underline x_2^2]$ & $\frac{-c_1}{\sqrt{c_1^2+c_2^2}}R$ & $\frac{-c_2}{\sqrt{c_1^2+c_2^2}}R$ & $-R\sqrt{c_1^2+c_2^2}$\\
&- & - & $[\frac{c_1^2+c_2^2}{c_2^2}\underline x_2^2, \underline x_1^2+\underline x_2^2]$ & $-\sqrt{R^2-\underline x_2^2}$ & $\underline x_2$ & $c_2 \underline x_2- c_1\sqrt{R^2-\underline x_2^2}$\\
\hline

$(\underline x_1,\underline x_2)$,$(\overline x_1,\overline x_2)$,$(\overline x_1,\underline x_2)$&- & - & $[\overline x_1^2+\overline x_2^2,\overline x_1^2+\underline x_2^2]$ & $\overline x_1$ & $-\sqrt{R^2-\overline x_1^2}$ & $c_1\overline x_1-c_2\sqrt{R^2-\overline x_1^2}$\\
&- & - & $[\overline x_1^2+\underline x_2^2], \underline x_1^2+\underline x_2^2]$ & $-\sqrt{R^2-\underline x_2^2}$ & $\underline x_2$ & $c_2 \underline x_2- c_1\sqrt{R^2-\underline x_2^2}$\\
\hline

&- & + & $[\overline x_1^2+\underline x_2^2,\underline x_1^2+\underline x_2^2]$ & $-\sqrt{R^2-\underline x_2^2}$ &$\underline x_2$ & $c_2 \underline x_2- c_1\sqrt{R^2-\underline x_2^2}$ \\
\hline
&+ & - & $[\underline x_1^2+\overline x_2^2,\underline x_1^2+\underline x_2^2]$ &$\underline x_1$ & $-\sqrt{R^2-\underline x_1^2}$ & $c_1 \underline x_1- c_2\sqrt{R^2-\underline x_1^2}$ \\
\hline
&+ & + & Whatever & $\underline x_1$ & $\underline x_2$ & $c_1\underline x_1+c_2\underline x_2$ \\
\hline
\end{tabular}
\end{center}
\label{tab:objf1R}
\end{table}

\begin{lemma}
Let $h(x)=a R^2-c\sqrt{R^2-b}$. Then its unique minimizer on $[R_1,R_2]\in \mathbb{R}$ is $R=[\sqrt{b+\frac{c^2}{4a^2}}]_{R_1}^{R_2}$.
\end{lemma}
\begin{lemma}
Let $h(x)=a R^2-cR$. Then its unique minimizer on $[R_1,R_2]\in \mathbb{R}$ is $R=[c/2a]_{R_1}^{R_2}$.
\end{lemma}
\begin{lemma}
Let $h(x)=a R-cR$. Then its unique minimizer on $[R_1,R_2]\in \mathbb{R}$ is $\min\{(a-c)R_1,(a-c)R_2\}$.
\end{lemma}
\begin{lemma}
Let $h(x)=a R-c\sqrt{R^2-b}$. Then its unique minimizer on $[R_1,R_2]\in \mathbb{R}$ is $R=[\sqrt{ba^2/(a^2-c^2)}]_{R_1}^{R_2}$.
\end{lemma}

The algorithm developed turns out to be $1000$ times faster than generic CVX solver.

==> texcode/proposal2.tex <==
\section{Proposal}
\bi
\item Dual decomposition
\item ADMM: More message passing but likely less steps to converge.
\item Benders decomposition
\ei
\section{Case Study: 2 bus network}

Suppose there are two buses $0$ and $1$, the OPF problem then can be stated explicitly as:

\noindent OPF-1.0:
\bqn
\min && f_0(p_0)+f_1(p_1)\\
\text{s.t.}  && v_1=v_0-2(r_0P_0+x_0Q_0)+\ell_0 |z_0|^2\\
&& p_0=P_0\\
              && p_1=-(P_0-\ell_0 r_0)\\
&& q_0=Q_0\\
&& q_1=-(Q_0-\ell_0 x_0)\\
&& v_0\ell_0\geq P_0^2+Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline v_1\leq v_1\leq \overline v_1\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline p_1\leq p_1\leq \overline p_1\\
&& \underline q_0\leq q_0\leq \overline q_0\\
&& \underline q_1\leq q_1\leq \overline q_1
\eqn

\subsection{Dual Decomposition}
\qiuyu{The dual decomposition  does not convergence unless the objective is strictly convex in $p,q,v,\ell$, which is hardly satisfied.}



Let $\hat S_0:=S_0$ and $\tilde S_0:=S_0-\ell_0 z_0$ as local copies, OPF-1.0 can be rewritten equivalently as:

\noindent OPF-1.1:
\bqn
\min && f_0(p_0)+f_1(p_1)\\
\text{s.t.} && \hat P_0=\tilde P_0-\ell_0 r_0\\
               && \hat Q_0=\tilde Q_0-\ell_0 x_0\\
               && v_1=v_0-2(r_0\hat P_0+x_0\hat Q_0)+\ell_0 |z_0|^2\\
&& p_0=\hat P_0\\
              && p_1=-\tilde P_0\\
&& q_0=\hat Q_0\\
&& q_1=-\tilde Q_0\\
&& v_0\ell_0\geq \hat P_0^2+\hat Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline v_1\leq v_1\leq \overline v_1\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline p_1\leq p_1\leq \overline p_1\\
&& \underline q_0\leq q_0\leq \overline q_0\\
&& \underline q_1\leq q_1\leq \overline q_1
\eqn

We relax the first three constraints with multipliers $\lambda_1,\lambda_2,\lambda_3$ and OPF-1.2 can be rewritten equivalently as:

\noindent OPF-1.2:
\bqn
\max_{\lambda} \quad g(\lambda)
\eqn
where 
\bqn
g(\lambda):=\min_{x} && f_0(p_0)+f_1(p_1)+\lambda_1(\hat P_0-\tilde P_0+\ell_0 r_0)+\lambda_2(\hat Q_0-\tilde Q_0+\ell_0 x_0)+\lambda_3(v_1-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)\\
\text{s.t.} 
&& p_0=\hat P_0\\
              && p_1=-\tilde P_0\\
&& q_0=\hat Q_0\\
&& q_1=-\tilde Q_0\\
&& v_0\ell_0\geq \hat P_0^2+\hat Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline v_1\leq v_1\leq \overline v_1\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline p_1\leq p_1\leq \overline p_1\\
&& \underline q_0\leq q_0\leq \overline q_0\\
&& \underline q_1\leq q_1\leq \overline q_1
\eqn
The subproblem corresponding to bus $0$ is 

\noindent OPF-bus0-1.0:
\bqn
\min_{x} && f_0(p_0)+\lambda_1(\hat P_0+\ell_0 r_0)+\lambda_2(\hat Q_0+\ell_0 x_0)+\lambda_3(-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)\\
\text{s.t.} 
&& p_0=\hat P_0\\
&& q_0=\hat Q_0\\
&& v_0\ell_0\geq \hat P_0^2+\hat Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline q_0\leq q_0\leq \overline q_0
\eqn
or 

\noindent OPF-bus0-1.1:
\bqn
\min_{x} && f_0(p_0)+\lambda_1(p_0+\ell_0 r_0)+\lambda_2( q_0+\ell_0 x_0)+\lambda_3(-v_0+2(r_0 p_0+x_0 q_0)-\ell_0 |z_0|^2)\\
\text{s.t.} 
&& v_0\ell_0\geq  p_0^2+ q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline q_0\leq q_0\leq \overline q_0
\eqn
If $f_0(p_0)$ is linear in $p_0$, then OPF-bus0-1.1 is a LQP of the following form:


\subsection{ADMM}

Radial network is a bipartite graph, which suggests a very good decomposition using ADMM. We will still use the 2 bus network as an example.
Let $\hat S_0:=S_0$ and $\tilde S_0:=S_0-\ell_0 z_0$ as local copies, as done in OPF-1.1. We relax the first three constraints with multipliers $\lambda_1,\lambda_2,\lambda_3$ and OPF-2.1 can be rewritten equivalently as:

\noindent OPF-1.2:
\bqn
\max_{\lambda} \quad g(\lambda)
\eqn
where 
\bqn
g(\lambda):=\min_{x} && f_0(p_0)+f_1(p_1)+\lambda_1(\hat P_0-\tilde P_0+\ell_0 r_0)+\lambda_2(\hat Q_0-\tilde Q_0+\ell_0 x_0)+\lambda_3(v_1-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)\\
&& + \frac{\rho}{2}(v_1-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)^2\\
\text{s.t.} 
&& p_0=\hat P_0\\
              && p_1=-\tilde P_0\\
&& q_0=\hat Q_0\\
&& q_1=-\tilde Q_0\\
&& v_0\ell_0\geq \hat P_0^2+\hat Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline v_1\leq v_1\leq \overline v_1\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline p_1\leq p_1\leq \overline p_1\\
&& \underline q_0\leq q_0\leq \overline q_0\\
&& \underline q_1\leq q_1\leq \overline q_1
\eqn

The subproblem at bus $0$ is ($v_1$ is given)

\noindent OPF-bus0-2.0:
\bqn
\min_{x} && f_0(p_0)+\lambda_1(\hat P_0+\ell_0 r_0)+\lambda_2(\hat Q_0+\ell_0 x_0)+\lambda_3(-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)+ \frac{\rho}{2}(v_1-v_0+2(r_0\hat P_0+x_0\hat Q_0)-\ell_0 |z_0|^2)^2\\
\text{s.t.} 
&& p_0=\hat P_0\\
&& q_0=\hat Q_0\\
&& v_0\ell_0\geq \hat P_0^2+\hat Q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline q_0\leq q_0\leq \overline q_0
\eqn
or 

\noindent OPF-bus0-2.1:
\bqn
\min_{x} && f_0(p_0)+\lambda_1(p_0+\ell_0 r_0)+\lambda_2( q_0+\ell_0 x_0)+\lambda_3(-v_0+2(r_0 p_0+x_0 q_0)-\ell_0 |z_0|^2)+ \frac{\rho}{2}(v_1-v_0+2(r_0p_0+x_0q_0)-\ell_0 |z_0|^2)^2\\
\text{s.t.} 
&& v_0\ell_0\geq  p_0^2+ q_0^2\\
&& \underline v_0\leq v_0\leq \overline v_0\\
&& \underline p_0\leq p_0\leq \overline p_0\\
&& \underline q_0\leq q_0\leq \overline q_0
\eqn
If $f_0(p_0)$ is linear in $p_0$, then OPF-bus0-1.1 is a LQP of the following form:
\bqn
\min && \sum_{i=1}^4 c_ix_i+\frac{\rho}{2}(\sum_{i=1}^4d_ix_i+d_5)^2\\ 
\text{s.t.}&&\underline x_i \leq  x_i\leq \overline x_i \ \ 1\leq i\leq 4 \\
&& x_3x_4\geq x_1^2+x_2^2
\eqn

Let $y_1=x_1$, $y_2=x_2$, $y_3=(x_3-x_4)/2$ and $y_4=(x_3+x_4)/2$, the above problem has the following form:
\bqn
\min && \sum_{i=1}^4 c'_iy_i+\frac{\rho}{2}(\sum_{i=1}^4d'_iy_i+d'_5)^2\\ 
\text{s.t.}&&\underline x_i \leq  y_i\leq \overline x_i \ \ 1\leq i\leq 2 \\
&&  \underline x_3 \leq   y_3+y_4\leq \overline x_3\\
&&  \underline x_4 \leq  y_4-y_3 \leq \overline x_4\\
&& y\in SOC(\mathbf{R}^4)
\eqn


\subsection{Modified ADMM \& Dual Decomposition}

It turns out that most of the constraints are local, thus is unnecessary to relax.













==> texcode/proposal3.tex <==

\section{Distributed Algorithm for OPF}\label{sec:alg}

We assume SOCP relaxation is exact and  develop in this section
a distributed algorithm that solves ROPF. 
We first review a standard alternating direction method of multiplier (ADMM).
We then make use of the structure of ROPF to speed up the standard ADMM algorithm 
by deriving close form expressions for the optimization subproblems in each ADMM iteration.


\subsection{Preliminary: ADMM}

ADMM blends the decomposability of dual decomposition with the superior convergence properties of the method of multipliers
\cite{boyd2011distributed}. It solves optimization problem of the form:
\bq
\min_{x,z} && f(x)+g(z) \nonumber \\
\text{s.t.} && x\in\mathcal{K}_x, \ \ z\in\mathcal{K}_z \label{eq:admm}\\
&& Ax+Bz=c \nonumber
\eq
where $\mathcal{K}_x,\mathcal{K}_z$ are convex sets. Let $\lambda$ denote the Lagrange
 multiplier for the constraint $Ax+Bz=c$.   Then the augmented Lagrangian is defined as
\bqn
L_\rho(x,z,\lambda)&:=&f(x)+g(z)+\lambda^T(Ax+Bz-c)\\
&&+\frac{\rho}{2}\|Ax+Bz-c\|^2,
\eqn
where  $\rho\geq 0$ is a constant. When $\rho=0$, the augmented Lagrangian reduces to 
the standard Lagrangian. ADMM consists of the iterations:
\begin{subequations}\label{eq:update}
\bq
x^{k+1}&\in&\arg\min_{x\in\mathcal{K}_x} L_\rho(x,z^{k},\lambda^k)\label{eq:xupdate}\\
z^{k+1}&\in&\arg\min_{z\in\mathcal{K}_z} L_\rho(x^{k+1},z,\lambda^k)\label{eq:zupdate}\\
\lambda^{k+1}&=&\lambda^{k}+\rho(Ax^{k+1}+Bz^{k+1}-c)\label{eq:mupdate}
\eq
\end{subequations}
Compared to dual decomposition, ADMM is guaranteed to converge to an optimal 
solution under less restrictive conditions. Let
\begin{subequations}\label{eq:feasible}
\bq
r^k&:=&\|Ax^k+Bz^k-c\| \label{eq:pfeasible}\\
s^k&:=&\rho\|A^TB(z^{k}-z^{k-1})\| \label{eq:dfeasible}
\eq
\end{subequations}
They can be viewed as the residuals for primal and dual feasibility.
Assume: 
\bi
\item A1: $f$ and $g$ are closed proper and convex.
\item A2: The unaugmented Lagrangian $L_0$ has a saddle point.
\ei
The correctness of ADMM is guaranteed by the following result 
in \cite[Chapter 3]{boyd2011distributed}.
\begin{proposition}[\cite{boyd2011distributed}]
Suppose A1 and A2 hold. Let $p^*$ be the optimal objective value.  
% and $p^k:=f(x^k)+g(z^k)$.
Then 
\bqn
\lim_{k\rightarrow \infty}r^k=0,  \quad  \lim_{k\rightarrow \infty}s^k=0
\eqn
implying
\bqn
\lim_{k\rightarrow \infty} f(x^k)+g(z^k)= p^*
\eqn
\end{proposition}

\subsection{Decoupling in ADMM}\label{sec:application}

In applying ADMM to ROPF, we first exploit the structure of ROPF to derive
subproblems that are decoupled and can be solved concurrently.  We then 
derive closed form solutions to these subproblems.  In this subsection we explain
how the standard technique of decoupling through local variables.

Consider the problem:
\begin{subequations}\label{eq:admm_app}
\bq
\min_{x\in \mathbb R^n} && f(x) \label{eq:admm_app1} \\
\text{s.t.} &&    a_i^Tx=b_i, \ \ i\in \mathI  \label{eq:admm_app2}\\
&& x\in  \mathcal{K}_z \label{eq:admm_app3}
\eq
\end{subequations}
where $f(x)$ is a convex function and $\mathcal{K}_z \subseteq \mathbb R^n$ is a convex set. 
Suppose we 
Let $\{\mathI_l,1\leq l\leq m\}$ be a partition of $\mathI$, i.e. $\cup_{1\leq l\leq m}\mathI_l=\mathI$, and 
\bqn
\mathcal{K}_x:=\cup_{l=1}^m\{x^{(l)}\mid a_i^Tx^{(l)}=b_i, i\in\mathI_l \}
\eqn
then \eqref{eq:admm_app} is equivalent to 
\bq
\min_{x,z} && f(z)\nonumber\\
\text{s.t.}&& x\in\mathcal{K}_x,  \ \ z\in \mathcal{K}_z \label{eq:admm_app4}\\
&& x^{(l)}-z=0 \quad   1 \leq  l\leq m \nonumber
\eq
where $x:=\{x^{(l)},1\leq l\leq m\}$. Relax the last equality for each $l$ and the augmented Lagrangian is 
{\small
\bqn
L_\rho(x,z,\lambda):=f(z)+\sum_{l=1}^{m}\left( (\lambda^{(l)})^T(x^{(l)}-z)+\frac{\rho}{2}\|x^{(l)}-z\|^2\right)
\eqn}
Then we can update the primal variables $(x,z)$ and the multipliers $\lambda$ according to \eqref{eq:update}.

The purpose of the partition of the index set $\mathI$ is to make the constraints in \eqref{eq:admm_app2} local, i.e. the update in \eqref{eq:update} can be decomposed into several small optimization subproblems that can be solved simultaneously. Next, we will show that two partitions are sufficient for designing distributed OPF algorithm using this approach.

\subsection{Distributed OPF algorithm}

In this section, we apply the decomposition approach described in section \ref{sec:application} to develop a distributed algorithm that solves ROPF \eqref{eq:ropf}. The advantages of the proposed algorithm are
\bi
\item For each agent\footnote{Each bus is an agent.}, we solve its corresponding subproblem efficiently, i.e. we derive a close form expression for each optimization subproblem, which is usually solved by iterative algorithms:\cite{lam2012optimal,lam2012distributed,dall2012distributed,sun2013fully,devane2013stability,li2012demand,kim1997coarse,baldick1999fast}.
\item Communication is only required between adjacent buses.
\ei
We can write the ROPF problem \eqref{eq:ropf} in the form of \eqref{eq:admm_app} as sequel.
\bqn
\min_{x}&& \sum_{i\in \mathN}f_i(p_i,\ell_i)\\
\text{s.t.} && x \text{ satisfies } \eqref{eq:bfm1}-\eqref{eq:bfm3}\\
&& x\in\mathcal{K}_z
\eqn
where $\mathcal{K}_z:=\{z\mid z \text{ satisfies \eqref{eq:operation} and \eqref{eq:bfm5}} \}$. Next, we will partition the constraints in \eqref{eq:bfm1}-\eqref{eq:bfm3} to write it equivalently in the form of \eqref{eq:admm_app4} such that the update in \eqref{eq:update} can be done simultaneously by each agent. 

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{figure/tree.png}
\caption{Example of a graph with tree topology.}
\label{fig:tree}
\end{figure}

We assume each bus $i\in\mathN$ is an agent with its local variables $x_i:=(v_i,\ell_i,P_i,Q_i,p_i,q_i)$. Then the constraints in $\mathK_z$ are local, i.e. they are separable for each agent $i$. Note that the network $\mathT$ is a tree, which is a bipartite graph and can be partitioned into two groups $\mathI_1:=\{i\in\mathN\mid i \text{ is in the odd layer}\}$ and $\mathI_2:=\{i\in\mathN\mid i \text{ is in the even layer}\}$. For instance, there are four layers in Fig. \ref{fig:tree} and $\mathI_1=\{1,4,5,6\}$ and $\mathI_2=\{2,3,7,8,9\}$. Let 
\bqn
\mathcal{K}_x=\cup_{l=1}^2\{x_i^{(l)}\mid x_i^{(l)} \text{ satisfies \eqref{eq:bfm1}-\eqref{eq:bfm3} for }i\in\mathI_l\}
\eqn

Under such partition, bus $i\in \mathI_1$ ($\mathI_2$) is only coupled with buses $k\in \mathI_2$ ($\mathI_1$). In particular, by \eqref{eq:bfm1}, each bus $i$ needs the voltage $v_{A_i}$ from its ancestor $A_i$, thus we create a copy $v_{A_i,i}$, representing the replication of $v_{A_i}$ at bus $i$. On the other hand, in \eqref{eq:bfm2} and \eqref{eq:bfm3}, each bus $i$ needs $\ell_j,P_j,Q_j$ from all of its children $j\in C_i$ and we create a copy $\ell_{j,i},P_{j,i},Q_{j,i}$ of each $j\in C_i$ at bus $i$. Then the ROPF problem \eqref{eq:ropf} can be written in the form of \eqref{eq:admm_app4}.

\noindent E-ROPF:
\begin{subequations}\label{eq:mropf}
\small
\begin{align}
\min_{x} \ \ & \sum_{i\in\mathN}f_i(p_i^{(z)},\ell_i^{(z)}) \nonumber\\
\mathrm{s.t.}\ \ &v_{A_i,i}^{(l)}=v_i^{(l)}-2(r_i P_i^{(l)}+x_iQ_i^{(l)})+\ell_{i}^{(l)}(r_i^2+x_i^2) \ \ i\in \mathE  \label{eq:d1}\\  
& \sum_{j\in C_i}(P_{j,i}^{(l)}-\ell_{j,i}^{(l)}r_{j})+p_i^{(l)}=P_{i}^{(l)} \ \ i\in \mathN  \label{eq:d2}\\  
& \sum_{j\in C_i}(Q_{j,i}^{(l)}-\ell_{j,i}^{(l)}x_{j})+q_i^{(l)}=Q_{i}^{(l)} \ \ i\in \mathN  \label{eq:d3}\\  
& (P_i^{(z)})^2+(Q_i^{(z)})^2\leq v_i^{(z)}\ell_{i}^{(z)} \ \ i\in\mathE  \label{eq:d4}\\
& (p_i^{(z)},q_i^{(z)})\in\mathcal{S}_i  \ \ i\in\mathN  \label{eq:d5}\\
& \underline v_i\leq  v_i^{(z)}\leq \overline v_i \ \ i\in\mathN \label{eq:d6}\\
& x^{(l)}-z=0 \ \ l\in\{1,2\} \label{eq:d7}
\end{align}
\end{subequations}
where \eqref{eq:d1}-\eqref{eq:d3} form $\mathK_x$ and $\eqref{eq:d4}-\eqref{eq:d6}$ form $\mathK_z$. The value of the superscript $l$ depends on the partition that $i$ belongs to, i.e. $l=1$ ($2$) if $i\in\mathI_1$ ($\mathI_2$). Let $\lambda$, $\gamma$ and $\mu$ be Lagrangian multipliers associated with $x^{(l)}-z=0$, in particular 

\vspace{0.05in}

\begin{tabular}{|c|c||c|c|}
\hline
$\lambda_{1,i}$: & $v_i^{(l)}-v^{(z)}_i=0$ & $\lambda_{2,i}$: & $\ell_i^{(l)}-\ell^{(z)}_i=0$\\
\hline
$\lambda_{3,i}$: & $P_i^{(l)}-P^{(z)}_i=0$ & $\lambda_{4,i}$: & $Q_i^{(l)}-Q^{(z)}_i=0$\\
\hline
$\lambda_{5,i}$: & $p_i^{(l)}-p^{(z)}_i=0$ & $\lambda_{6,i}$: & $q_i^{(l)}-q^{(z)}_i=0$\\
\hline
$\mu_{1,i}$: & $\ell_{i,A_i}^{(l)}-\ell_{i}^{(z)}=0$ & $\mu_{2,i}$: & $P_{i,A_i}^{(l)}-P_{i}^{(z)}=0$ \\
\hline
$\mu_{3,i}$: & $Q_{i,A_i}^{(l)}-Q_{i}^{(z)}=0$ & &\\ 
\hline
$\gamma_j$: & \multicolumn{3}{|c|}{$v_{i,j}^{(l)}-v_{i}^{(z)}=0$ for $j\in C_i$} \\
\hline
\end{tabular}
Denote
\bqn
x^{(l)}_i&:=&(v_i^{(l)},\ell_i^{(l)},P_i^{(l)},Q_i^{(l)},p_i^{(l)},q_i^{(l)})\\
z_i&:=&(v^{(z)}_i,\ell^{(z)}_i,P^{(z)}_i,Q^{(z)}_i,p^{(z)}_i,q^{(z)}_i)\\
x^{(l)}_{i,A_i}&:=&(\ell_{i,A_i}^{(l)},P_{i,A_i}^{(l)},Q_{i,A_i}^{(l)})\\
\lambda_i&:=& (\lambda_{k,i}\mid k=1,2,3,4,5,6)\\
\mu_i &:=&  (\mu_{k,i}\mid k=1,2,3)
\eqn
Then the variables maintained by each bus (agent) $i$ is given below.
\bqn
\mathcal{A}_i:=\{x^{(l)}_i, x_{i,A_i}^{(l)}, \{v^{(l)}_{i,j},\gamma_j\mid j\in C_i\}, z_i,\lambda_i,\mu_i,\}.
\eqn


\begin{figure*}
\begin{subequations}\label{eq:AL}
%\footnotesize
\scriptsize
\begin{align}
&L_{\rho}(x,z,\lambda,\gamma,\mu)\label{eq:AL1}\\
=&\sum_{i\in\mathN}\left(f_i(p_i^{(z)})+\lambda_i^T(x^{(l)}_i-z_i)+\mu_i^T(x^{(l)}_{i,A_i}-z_i)+\sum_{j\in C_i}\gamma_j(v_{i,j}^{(l)}-v_{i}^{(z)})+\frac{\rho}{2}\left(\|x^{(l)}_i-z_i\|^2 + \|x^{(l)}_{i,A_i}-z_i\|^2+\sum_{j\in C_i}(v_{i,j}^{(l)}-v_{i}^{(z)})^2 \right)\right)\label{eq:AL2}\\
=&\sum_{i\in\mathN}\left(f_i(p_i^{(z)})+\lambda_i^T(x^{(l)}_i-z_i)+\sum_{j\in C_i}\mu_j^T(x^{(l)}_{j,i}-z_j)+\gamma_i(v_{A_i,i}^{(l)}-v_{A_i}^{(z)})+\frac{\rho}{2}\left(\|x^{(l)}_i-z_i\|^2 + \sum_{j\in C_i}\|x^{(l)}_{j,i}-z_j\|^2+(v_{A_i,i}^{(l)}-v_{A_i}^{(z)})^2 \right)\right)\label{eq:AL3}
\end{align}
\end{subequations}
\hrulefill
\end{figure*}

Next, we demonstrate that the E-ROPF problem \eqref{eq:mropf} can be solved in a distributed manner, i.e. both the $x$-update \eqref{eq:xupdate} and $z$-update \eqref{eq:zupdate} can be decomposed into small subproblems that can be solved simultaneously. For ease of presentation, we remove the iteration number $k$ in \eqref{eq:update} for all the variables, which will be updated accordingly after each subproblem is solved. The augmented Lagrangian for modified ROPF problem is given in \eqref{eq:AL}. We abuse notations in \eqref{eq:AL} and denote $x^{(l)}_{i,A_i}-z_i:=(\ell_{i,A_i}^{(l)}-\ell_i^{(z)},P_{i,A_i}^{(l)}-P_i^{(z)},Q_{i,A_i}^{(l)}-Q_i^{(z)})$ although there are 3 entries in $x^{(l)}_{i,A_i}$ but 6 entries in $z_i$. By \eqref{eq:AL3}, in the x-update step \eqref{eq:xupdate}, we solve
\bqn
\arg\min_{x\in\mathK_x}L_\rho(x,z,\lambda,\gamma,\mu)=\arg\min_{x\in\mathK_x}\sum_{i\in\mathN}G_i(x^{(l)}),
\eqn
where 
\begin{align*}
&G_i(x^{(l)}):=\lambda_i^Tx^{(l)}_i+\sum_{j\in C_i}\mu_j^Tx_{j,i}^{(l)}+\gamma_iv_{A_i,i}^{(l)}+\\
&\frac{\rho}{2}\left(\|x^{(l)}_i-z_i\|^2+\sum_{j\in C_i}\|x_{j,i}^{(l)}-z_j\|^2+(v_{A_i,i}^{(l)}-v_{A_i}^{(z)})^2\right)
\end{align*}
For each agent $i$, the corresponding subproblem is 
\begin{align}
\min \ & G_i(x^{(l)})\label{eq:algx}\\
 \text{s.t.} \ &\ v_{A_i,i}^{(l)}=v_i^{(l)}-2(r_iP_{i}^{(l)}+x_iQ_{i}^{(l)})+\ell_{i}^{(l)}(r_i^2+x_i^2) \nonumber\\%\\  
& \sum_{j\in C_i}(P^{(l)}_{j,i}-\ell^{(l)}_{j,i}r_{j})+p_i^{(l)}=P_{i}^{(l)} \nonumber\\
& \sum_{j\in C_i}(Q^{(l)}_{j,i}-\ell^{(l)}_{j,i}x_{j})+q_i^{(l)}=Q_{i}^{(l)} \nonumber
\end{align}
which takes the following form 
\bq
\min_x \ \ \frac{\rho}{2}\|x\|_2^2+c^Tx \quad \text{s.t. } Bx=0  \label{eq:xupdate1}
\eq
whose close form solution is given as 
\bqn
x=\frac{1}{\rho}(B^T(BB^T)^{-1}Bc-\frac{1}{\rho}c
\eqn
%\bqn
%x=B^T(BB^T)^{-1}(\frac{1}{\rho}Bc+d)-\frac{1}{\rho}c
%\eqn
Prior to perform the update, each agent $i$ needs to request variables from its parent $A_i$ and children $j\in C_i$. In particular, it needs to get $v_{A_i,i}^{(l)}$, $v_{A_i}^{(z)}$ and $\gamma_i$ from its ancestor $A_i$ and $x_{j,i}^{(l)},z_{j},\mu_j$ from all of its children $j\in C_i$. After the update, it needs to send the updated variables back to its ancestor $A_i$ and its children $j\in C_i$. The communication is illustrated in figure \ref{fig:xupdate}. 

\begin{figure}
\centering
\subfloat[Data received by agent $i$ before the $x$-update.] {
	\includegraphics[scale=0.22]{figure/x_update1.png}
	\label{fig:x_update1}
	}
\subfloat[Data sent by agent $i$ after the $x$-update.]{
	\includegraphics[scale=0.22]{figure/x_update2.png}
	\label{fig:x_update2}
	}
\caption{The communications in $x$-update step.}
\label{fig:xupdate}
\end{figure}

 Based on \eqref{eq:AL2}, In the $z$-update step, we solve
\bqn
\arg\min_{z\in\mathK_z}L_\rho(x,z,\lambda,\gamma,\mu)=\arg\min_{z\in\mathK_z}\sum_{i\in\mathN}H_i(z),
\eqn
where 
\begin{align*}
&H_i(z):=f(p_i^{(z)},\ell_i^{(z)})-\lambda_i^Tz_i-\mu_i^Tz_i-\sum_{j\in C_i}\gamma_jv_i^{(z)}+\\
&\frac{\rho}{2}\left(\|x^{(l)}_i-z_i\|^2 + \|x^{(l)}_{i,A_i}-z_i\|^2+\sum_{j\in C_i}(v_{i,j}^{(l)}-v_{i}^{(z)})^2 \right)
\end{align*}
The subproblem solved by each agent $i$ is 
\bqn
\min && H_i(z)\label{eq:algz}\\
\text{s.t.}&&   (P^{(z)}_{i})^2+(Q^{(z)}_{i})^2 \leq v^{(z)}_i\ell^{(z)}_{i} \\
&& \underline v_i\leq v^{(z)}_i\leq \overline v_i\nonumber\\
&& (p_i^{(z)},q_i^{(z)})\in \mathcal{S}_i
\eqn
Suppose $f_i(p_i^{(z)},\ell_i^{(z)})$ is linear or quadratic over its argument, let $k=(|C_i|+1)^{-\frac{1}{2}}$ and scale $v_i^{(k)}$ down by $k$ in the above problem, then it takes the following form:

 \bq\label{eq:ab1}
\min_y && \sum_{i=1}^6(y_i^2+c_iy_i) \\
\text{s.t. } && y_1^2+y_2^2\leq k^2 y_3y_4  \nonumber\\
&& \underline y_3 \leq y_3\leq \overline y_3 \nonumber\\
&& (y_5,y_6)\in \mathcal{S}_i \nonumber
\eq
Note that $(y_1,\dots,y_4)$ and $(y_5,y_6)$ are independent in the optimization problem \eqref{eq:ab1}, thus we have two independent subproblems. The first subproblem solves
\bq
\min_{y_5,y_6} \  \sum_{i=5}^6(y_i^2+c_iy_i) \text{ s.t. }  (y_5,y_6)\in\mathS_i\nonumber
\eq
which determines the update of $(y_5,y_6)$. If the feasible set $\mathS_i$ takes the form of \eqref{eq:S1}, the close form solution is
\bqn
(y_5,y_6)=-\frac{1}{2}\min\{1,\frac{2\overline s_i}{\sqrt{c_1^2+c_2^2}}\}(c_5,c_6)
\eqn
If the feasible set $\mathS_i$ takes the form of \eqref{eq:S2}, the close form solution is
\bqn
(y_5,y_6)=(\left[\frac{-c_5}{2}\right]_{\underline p_i}^{\overline p_i}, \left[\frac{-c_6}{2}\right]_{\underline q_i}^{\overline q_i}),
\eqn
where $[x]_a^b:=\min\{b,\max\{x,a\}\}$. The second subproblem solves
 \bqn
\min_{y_1,y_2,y_3,y_4} && \sum_{i=1}^4(y_i^2+c_iy_i) \\
\text{s.t. } && y_1^2+y_2^2\leq k^2 y_3y_4  \\
&& \underline y_3 \leq y_3\leq \overline y_3
\eqn
which determines the update of $(y_1,\dots,y_4)$. In Appendix \ref{app:solver2}, we show the procedure of how to obtain close form expressions for this problem. After the z-update step, we update the Lagrangian multipliers for the relaxed constraints as \eqref{eq:mupdate}. Both the z-update and multiplier update steps only involve variables within the agent and no communication is required.

Finally, we will specify the stopping criteria for the algorithm. Empirical results show that the the solution is accurate enough when both the primal residual $r^k$ defined in \eqref{eq:pfeasible} and the dual residual $s^k$ defined in \eqref{eq:dfeasible} are below $10^{-4}\sqrt{N}$, where $N$ is the number of buses. The pseudo code for the algorithm is summarized in Table \ref{tab:alg}.
\begin{table}[htdp]
\caption{Distributed algorithm of OPF}
\centering
\begin{tabular}{|p{8cm}|}
\hline
{\bf Distributed Algorithm of OPF}\\
\hline
{\bf Input}: Network $\mathT$, Power injection region $\mathS_i$, Voltage region $(\underline v_i,\overline v_i)$,\\
\hspace{0.6cm} Line impedance $z_i$\\
{\bf Output}: Voltage $v$, Power injection $s$\\
\hline
1. Initialize the variables with any number. \\
2. Iterate the following step until both the primal residual $s^k$ \eqref{eq:pfeasible} and the dual residual $r^k$ \eqref{eq:dfeasible} are below $10^{-4}\sqrt{N}$.\\
\hspace{0.2cm} a. In the x-update, each agent $i$ solves \eqref{eq:algx} to update $x$.\\
\hspace{0.2cm} b. In the z-update, each agent $i$ solves \eqref{eq:algz} to update $z$.\\
\hspace{0.2cm} c. In the multipliers update, update the multiplier $\lambda,\mu,\gamma$ by  \eqref{eq:mupdate}.\\
\hline
\end{tabular}
\label{tab:alg}
\end{table}










